Security and Privacy Approaches in Mixed Reality: A Literature Survey

Mixed reality (MR) technology development is now gaining momentum due to advances in computer vision, sensor fusion, and realistic display technologies. With most of the research and development focused on delivering the promise of MR, there is only barely a few working on the privacy and security implications of this technology. This survey paper aims to put in to light these risks, and to look into the latest security and privacy work on MR. Specifically, we list and review the different protection approaches that have been proposed to ensure user and data security and privacy in MR. We extend the scope to include work on related technologies such as augmented reality (AR), virtual reality (VR), and human-computer interaction (HCI) as crucial components, if not the origins, of MR, as well as numerous related work from the larger area of mobile devices, wearables, and Internet-of-Things (IoT). We highlight the lack of investigation, implementation, and evaluation of data protection approaches in MR. Further challenges and directions on MR security and privacy are also discussed.

==> Devices_and_Platforms_survey.tex <==
\section{Mixed Reality Devices and Platforms}\label{sec:devices} %\section originally
The mixed reality pipeline
A generic MR processing pipeline is shown in Figure~\ref{fig:MRpipeline} which has three essential blocks: \textit{detection}, \textit{transformation}, and \textit{rendering}. Depending on the capabilities of the MR platform or device, the functionalities available can vary for each block. The detection focuses on gathering information such as user view orientation and direction, location, and surrounding objects. Thus, the detection process primarily depends on the sensing capabilities of the device. Early devices were limited to position or orientation sensors using magnetic fields, inertial measurement, or ultrasound. Now, GPS is widely used for location detection. Furthermore, vision-based techniques can be used to detect objects in the environment as well as the environment itself. After detection, the information gathered will be transformed or processed to deliver services. Depending on the service or application, different transformations are used. Finally, the results of the transformation is delivered to the user by rendering it through the device's output interfaces. Depending on the available output capabilities of the device, the result can be rendered as visual, auditory, or tactile. Therefore, in this section, we list some of the research prototypes and commercially available MR platforms and devices, and show their differences particularly in terms of detection and rendering capabilities. Although, we do not present a comprehensive listing of MR devices as it is not the goal of this survey; rather, we want to highlight how the platforms have advanced, and how security and privacy have been considered, if it was considered at all.


\subsection{Research Prototypes and Endeavours}\label{sec:prototypes}
The development of MR technology is totally-dependent on how human-computer interaction (HCI) has also developed. Early machines, i.e. computers, were task-specific, thus, most of these computers were designed to be task-assistants. Similarly, early MR devices were also extensions of these early task-centric computers. The purpose of MR was to bridge the physical space to the virtual space to allows users to interact with virtual objects, and early endeavours focused on creating platforms and interfaces to link the two spaces. Following the pipeline in Figure~\ref{fig:MRpipeline}, the subsequent subsections are grouped based on the rendering capabilities, i.e. the displays (Section~\ref{prototype:displays}), and detection capabilities, i.e. the user interfaces (Section~\ref{prototype:interfaces}). In addition, we also include the different MR-based collaboration prototypes (Section~\ref{prototype:collaborative}). Efforts on application-specific development, i.e. vehicular applications, are also covered.

\subsubsection{Mixed Reality Displays}\label{prototype:displays}
There are various display form factors that have been designed and used both for research and commercially-released MR platforms. Different use cases or applications called for different form factors. For personal MR applications, the near-eye displays, i.e. head-mounted displays or HMDs, and hand-held form factors were primarily used. Other use cases such as large-scale MR, or vehicular applications called for more appropriate form factors such as external projective technologies.

\paragraph{Head-mounted displays}
Since the very first near-eye head-mounted display \cite{sutherland1968head} was designed using miniature cathode ray tube displays and Boeing's use of an HMD to improve their manufacturing process using AR functionalities \cite{caudell1992augmented}, numerous HMDs have been released commercially and used for research. Boeing's demonstration used Reflection Technology's The Private Eye\footnote{Reflection Technology Private Eye, (Accessed 7 Sep 2017), https://www.google.com/culturalinstitute/beta/asset/reflection-technology-private-eye-display/QgFnZtDAdVz0CQ} which used an array of LEDs on its screen. The Private Eye has been utilised in other AR research demonstrations which combines it with head tracking devices to vary the displayed content depending on what the user is looking at \cite{feiner1993windows}. Other prototypes where designed for specific use cases such as the \textsc{EyeTap} \cite{mann2004continuous} which was used for continuous lifelogging or \textit{sousveillance}\footnote{Coined by Steve Mann to mean recording of an activity by a participant. This is in contrast to the concept of surveillance when activities are recorded by a non-participant or another entity such as government, security agencies, and so on.}. \textsc{EyeTap}'s latest iteration \cite{mann2013freeglass} now combines a 3D camera to provide more environmental sensing capabilities. All these HMDs mentioned above are see-through displays that allow augmentations within the user's field-of-view (FOV) at the same time allowing users to see their physical surroundings. Other near-eye display form factors, however, not really head-worn, includes the binoculars \cite{oskiper2015binoculars} which demands jitter-free tracking and precise augmentation. 

A different method based on retro-reflective projection have also been used in a head-mounted projective display (HMPD) prototype \cite{hua2005polarized}. Instead of creating an image near the eye, the HMPD creates the image by projecting it into a retro-reflective surface which, then, reflects the images back to the user's eyes. However, in order for it to be fully-immersive, the users have to be surrounded by these retro-reflective surfaces.

\paragraph*{Addressing challenges in MR HMD}Other research activities focused on the improvement of the rendering technology such as providing correct occlusion \cite{kiyokawa2003occlusion}, 3D sensor fusion for better environment modelling \cite{newcombe2011kinectfusion}, or augmentation in specular surfaces \cite{jachnik2012real}. Other addressed the issue of latency and tracking stability by reconstructing the environment on a video display (like a video see-through HMD) \cite{waegel2014reconstructive} \cite{benko2015fovear} \cite{xiao2016augmenting}

\paragraph{Hand-held displays}
Head-worn devices tend to be obtrusive and burdensome thus other use cases called for hand-held form factors. For example, the \textsc{ARPad} \cite{mogilev2002arpad} combines a camera, an LCD panel, and a 3D ball input device. Other hand-held MR demonstrations leveraged on the input and display capabilities of existing commercially available devices such as mobile phones \cite{mohring2004video} and tablets \cite{karlsson2012iar} to demonstrate see-through MR functionalities.

\paragraph{Other display form factors}
However, other use cases demanded hands-free and non-obtrusive displays. See-through desktop systems that were primarily designed for hands-free use cases include the \textsc{POLAR} \cite{olwal2005polar} and \textsc{ASTOR} \cite{olwal2005astor} prototypes. \textsc{POLAR}'s aim was to demonstrate a portable desktop AR using a half-silvered mirror to project images from a laptop computer display which will appear augmented on the objects put against the mirror. On the other hand, \textsc{ASTOR} uses two projectors and a holographic optical element (instead of a half-silvered mirror) to augment content stereoscopically. Both prototypes achieve optical see-through augmentations. Other prototype form factors were application-specific such as the vehicular use cases \cite{nakatsuru2003vehicle, sridhar2012vehicle, rao2014ar}.

There were also pure projection, i.e. non-see-through, prototypes that can transform any surface in to an MR display and/or interface. A wearable example of a camera-projector setup \cite{karitsuka2003wearable} has been demonstrated. Another example transforms an umbrella into an MR device \cite{hashimoto2007pileus} using a similar camera-projector setup with additional sensors (i.e. GPS, RFID reader, accelerometer, and compass). The \textsc{MirageTable} \cite{benko2012miragetable}, on the other hand, used a curved screen combined with a stereoscopic projector and camera to enable virtual and physical interactions in the same space. On the other hand, the \textsc{TeleAdvisor} \cite{gurevich2012teleadvisor} incorporates remote connectivity to a camera-projector setup to support remote assistance applications. Other projection setups such as \textsc{RoomAlive} \cite{jones2014roomalive} focused on delivering a large-scale MR environment using multiple projectors and depth cameras to transform an entire room into a gaming space.

\subsubsection{Interfaces}\label{prototype:interfaces}
Aside from creating platforms and devices, early research endeavours focused on designing user interfaces for MR. Early efforts include the tangible interfaces such as the \textsc{metaDESK}, \textsc{transBOARD}, and \textsc{ambientROOM} from MIT's Media Lab \cite{ishii1997tangible}, which they collectively call \textit{tangible bits} -- graspable and manipulable interfaces that are coupled with the digital information or ``bits''. These tangible bits are platforms that are composed of tangible interfaces, displays, and tracking devices that assists in the interaction of the physical and virtual space without the necessity for an HMD or other near-eye wearable displays. For example, the \textsc{metaDESK} uses lenses, and \textit{phicons} (or physical icons) that serve as tangible (physical) interface counterparts of graphical (virtual) interfaces such as display windows, and virtual icons respectively. Other examples of this tangible MR interface prototypes are the \textsc{MagicBook} \cite{billinghurst2001magicbook} which is a normal book but shows three-dimensional virtual images when viewed through an HMD, and the \textsc{MagicLens} \cite{looser2004through} which is used as a widget for zooming in and looking at details or features of an augmented virtual object. Similar interfaces have also been used for systems using retro-reflectivity \cite{brown2003widget} such as the HMPD described above.

In addition to these interfaces, many readily available devices have also been used as an MR input interface while using HMDs such as a smart phone \cite{budhiraja2013using} or a touch-enabled belt \cite{dobbelstein2015belt}. Additional efforts also focused on enabling 3D interactions on 2D touch interfaces \cite{wu2015touchsketch}, and providing tactile feedback \cite{sand2015head, kaul2016wearable} while using HMDs.

\subsubsection{Multi-user and Collaborative Platforms}\label{prototype:collaborative}
Aside from being an HCI medium or channnel, one of MR's early applications were as collaborative platforms. This was during an era when computers were not widely personal yet. \textsc{WearCom} \cite{billinghurst1999collaborative} was a collaborative MR platform which uses an HMD to allow remote collaborations through MR video conferencing, and co-located collaborations in a shared space. \textsc{WearCom}'s video conferencing application augments other participants around the user's field-of-view.  Similarly, \textsc{MagicMeeting} \cite{regenbrecht2002magicmeeting} provides a shared space co-located MR environment for collaborative 2D (through 2D display devices such as PDAs) and 3D (through an HMD) interactions. The Multi-user Augmented Reality Environment (or \textsc{MARE}) \cite{grasset2002mare} used a table top set up and focused on enabling natural human interactions with virtual objects. \textsc{Studierstube} \cite{schmalstieg2002} differentiates by having a distributed architecture for a more scalable collaborative MR. The distributed architecture of \textsc{Studierstube} reduces the processing and computation load through load-balancing, but requires resource migration to allow easy joining and exit of users. On the other hand, the \textsc{Scape} environment \cite{hua2004scape} uses retro-reflective surfaces and HMPDs, instead of the usual see-through HMDs as in \textsc{WearCom} or \textsc{Studierstube}. Other collaborative platform prototypes focused on how to virtually transport two remote users in the same shared MR space by rendering each of the user in front of the other user for face-to-face remote collaboration \cite{minatani2007face}. The main purpose of using MR in these collaborative platforms can be generalized in two points: to mediate between physical spaces of the users as well as between the physical and virtual spaces, and to serve as a communication channel in which users can exchange information across and within these spaces.

\subsubsection{Software Tool Kits, Systems, and Applications}

Behind these devices and platforms are software tool kits that have been especially developed to realize those functionalities. %One of the earliest were VR tool kits such as the \textsc{Minimal Reality} tool kit and the \textsc{DIVE}.
\textsc{Minimal Reality} \cite{shaw1993decoupled} is a VR tool kit developed for supporting VR interfaces in upcoming devices, and as a testbed or tool for VR applications as well as for investigating VR user interfaces. It is one of the earliest tool kits to address non-WIMP (windows, icons, menus, pointers) interfaces. DIVE \cite{carlsson1993dive}, on the other hand, is platform for multi-user VR application development using internet networking protocols. Other VR tool kits addresses other sub-problems such as the object-oriented framework \textsc{Avocado} \cite{tramberend1999avocado} which aims to improve communication in distributed VR, the \textsc{VRPN} \cite{taylor2001vrpn} which focuses on providing a uniform interface for heterogeneous VR devices, or the scalable peer-to-peer VR tool kit \textsc{Myriad} \cite{schaeffer2007myriad}.

For AR, one of the earliest and most well-known is the \textsc{ARToolKit} which was first developed in 1999 as a library of software tools\footnote{ARToolKit, (Accessed August 4, 2017), http://hitl.washington.edu/artoolkit/} for object detection and tracking. It was used in \textsc{MagicBook} \cite{billinghurst2001magicbook2} and was a popular choice for developing hand-held AR applications, e.g. using mobile phones with cameras \cite{wagner2003first}. \textsc{ARToolKit} is still continuously maintained and its latest version, ARToolKit6\footnote{ARToolKit6, (Accessed August 4, 2017),  https://artoolkit.org/}, is offered as an open source tracking and recognition SDK.

In general these SDKs follows the MR pipeline (shown in Figure ~\ref{fig:MRpipeline}) and, thus, the three processing blocks of detection, transformation, and rendering. For vision-based detection and rendering, there are generic and dedicated computer vision libraries such as the \textsc{OpenCV}, and 2D and 3D rendering tools such as the \textsc{OpenGL}. The ARToolKit's rendering block is based on \textsc{OpenGL}, while \textsc{OpenCV} libraries can be used with ARToolKit for object detection. The \textsc{Studierstube} system used a distributed version of the \textsc{Open Inventor}, which is based on OpenGL, to enable distributed 3D rendering in multi-user AR environments \cite{schmalstieg2000bridging}. Other early tool kits focused on improving the software work flow such as the \textsc{Tinmith-evo5} \cite{piekarski2003object} which is an object-oriented software architecture for MR applications similar to the \textsc{Avocado} VR system, while the \textsc{Morgan} framework \cite{ohlenburg2004morgan} provides an API for multi-user AR or VR projects. There are also projection-specific AR software architectures such as \textsc{ProjectedAugmentation2} \cite{ehnes2005projected}.

Current tool kits, such as \textsc{Wikitude}\footnote{wikitude, (Accessed August 4, 2017), https://www.wikitude.com/}, \textsc{Layar}\footnote{Layar, (Accessed August 4, 2017), https://www.layar.com/}, \textsc{EasyAR}\footnote{EasyAR, (Accessed August 4, 2017), https://www.easyar.com/}, and Apple's \textsc{ARKit}\footnote{ARKit - Apple Developer, (Accessed August 4, 2017), https://developer.apple.com/arkit/}, are now focused on application development and content creation. %The \textsc{Wikitude} SDK is one of the most widely used MR (specifically AR) SDKs with various original equipment manufacturers (OEM) using their SDK in developing MR applications. Both the \textsc{Wikitude} and \textsc{Layar} SDK have been primarily targeted for AR advertising, i.e. popping out 3D virtual objects using a mobile device's camera. The \textsc{ARKit} is the most recent of the three. It was unveiled by Apple at the Worldwide Developer's Conference (WWDC) 2017. This shows that Apple is joining the AR bandwagon by providing native support to AR functionalities on iOS devices
As a result, these tool kits are already used in numerous commercially available applications and devices. In the next section, we discuss the various commercially available MR devices and systems.

%table toolkits

These tool kits are now used to create MR applications on mobile devices and wearables. One of the most popular is the MR game Pokemon Go  \cite{pokemongo} that can augment pokemons, i.e. virtual pets, on the physical world as seen through a 2D touch screen on a mobile device. Another useful MR application is the image translation capability of the Google Translate \cite{googletranslate} which can read text on images and translate to supported languages.

Some of the currently available software tool kits, i.e. SDKs and/or APIs, are listed in Table~\ref{tab:toolkits}. Most of these tool kits are multi-platform (from ARToolkit down to Rox AR SDK) and are vision-based. Specifically, they are utilizing monocular (single vision) detection for 2D, 3D , and, for some, synchronous localization and mapping (or SLAM). Of these multi-platform, vision-based tool kits, only the ARToolkit is free and open source. Most of these paid tool kits have cloud support and are primarily focused on content and service creation, and application development. Furthermore, most of these tool kits, such as Wikitude, Layar, and Zapbox, are also shipped as platform applications that can be used to run other applications developed using the same tool kit.

On the other hand, there are also platform- and device-dependent tool kits listed. The ARkit is specifically for Apple's devices. The OSVR (Open Source Virtual Reality) is primarily for VR applications of specific smart glass devices, e.g HTC Vive and some Vuzix glasses, but can also be used for AR functionalities if devices have environment sensing capabilities such as front-facing cameras. The Meta 2 SDKs are obviously for the Meta 2 glasses. Similarly, the Windows MR APIs are for the Windows MR devices and the Hololens. These tool kits are primarily designed for the functionalities of these devices which includes other non-vision environmental sensing capabilities, e.g. depth sensing and head tracking, aside from the regular vision-based sensing. In the next section, we list the various commercially available MR devices, and include the tool kits  used for each one.

%Although most of the MR (VR and AR) applications now can be used with these accessories, there are also accessory-free MR applications or versions/modes of these applications, i.e. running 3D MR applications on 2D devices. The \textsc{Wikitude} \cite{wikitudesdk}, \textsc{Layar} \cite{layarsdk} SDK, and Apple's \textsc{ARKit} \cite{arkit} supports this accessory-free MR services.

%\subsubsection{A world-level mixed reality}
%%Remaining thrusts in MR technology: HCI and display.

\subsection{Commercially available Devices and Platforms}
Advances in hardware technology allowed MR devices to shrink in size and become more convenient to use especially the head-mounted and hand-held form factors. Furthermore, the processing, rendering, and camera power of non-MR specific devices such as smart phones and tablets allows them to instantly become MR-capable by just adding software (developed using any of the multi-platform SDKs listed in Table~\ref{tab:toolkits}) and/or hardware accessories such as stereoscopic goggles. We first take a look at these MR-enabling accessories and applications, and, then, proceed with the different MR-dedicated devices currently available in the market.

%% Please add the following required packages to your document preamble:
%% \usepackage{booktabs}

% table devices

\subsubsection{Accessory-enabled Mixed Reality}
Currently, the smart phone is still the primary mobile user device. Thus, most of the applications and hardware accessories now are designed for or around it. Excellent examples of these mobile-based devices are the head-worn goggle accessories such as the Samsung's Gear VR, and Google's Daydream and Cardboard accessories. %\cite{samsunggearVR} \cite{googledaydream} \cite{googlecardboard}
Content is displayed by the smart phone and is viewed through these accessories. Most content are primarily for 3D virtual experiences or VR. \textsc{Merge VR}\footnote{Merge VR, (Accessed Aug 4, 2017), https://mergevr.com/} is a transformable VR-AR accessory and supports both iPhone and Android smart phones. A Google cardboard-style MR accessory is also available, the \textsc{Zapbox}, which uses a see-through cardboard head-piece and tracking markers for easier real-world surface tracking and user interface detection \cite{zapbox}. The \textsc{Zapbox} also uses a marked cardboard wand as a user interface.

\subsubsection{Head-mounted devices}
Advances in display technology have given rise to the dedicated MR HMDs or collectively called as smart eye-wears. There are full-shut HMDs which are primarily for VR experiences as well as see-through HMDs for AR functionalities. The most popular VR headsets are the gaming headsets HTC Vive, Oculus Rift, and Sony Playstation VR \cite{vrheadsets}. These VR headsets are nearly full shut (prevents external light from bleeding in to the display), and provide hand-held controllers. The HTC Vive, however, has a font-facing camera which allows it to display synthetic content over the user's physical surroundings that allows it to be an AR device as well. These type of headsets are called video see-through HMDs which shows the augmentations as well as the environment in the same video display. This is in contrast to the optical see-through HMDs which utilises mirrors, lenses, holographic elements, and/or beam-splitters to create an image in the user's eyes which will seem augmented on the physical surrounding. Table~\ref{tab:devices} lists some commercially available HMDs.

\paragraph{Video see-through HMDs} These devices employs a video camera usually front-facing, as in the HTC Vive, to capture the environment, then, feed the video to a display propped in front of the user's field of view (FOV). Usually, the view of the user is blocked by the display device and the camera feed provides the front-facing view. Synthetic augmentations are then combined with the video feed. Various tool kits, such as the \textsc{Wikitude} SDK and \textsc{ARKit}, can be used for these video see-through HMDs. Thus, the \textsc{Zapbox}, and the \textsc{Merge VR} in AR mode are technically video see-through. Other dedicated video see-through HMDs are the Window's Mixed Reality devices manufactured by their partner original equipment manufacturers (OEM), e.g. Dell, HP, and Asus \cite{windowsmr}. These Windows MR devices are also nearly full shut, which makes these devices double as VR headsets, and have two front-facing cameras for stereo computer vision to enable AR mode.

There are also partly see-through devices such as the Recon Jet\footnote{Recon Jet, (Accessed 4 Aug 2017), https://www.reconinstruments.com/products/jet}, and the Vuzix M100/M300\footnote{Products, (Accessed 4 Aug 2017), https://www.vuzix.com/Products} smart glasses. These smart glasses uses a small enough video display positioned near one eye (usually on the right) so as not to block the user's FOV. These devices sprung from the wearable space and are, possibly, the most popularly known and widely used types of HMDs. Also, most of these devices perform very little to no object tracking which allows them to reduce processing and battery requirements, and, thus, reduce their size. These devices are usually linked to a smart phone and works as an additional display device to display notifications and content just like what a smart watch does nowadays.

\paragraph{Optical see-through HMDs}
On the other hand, optical see-through HMD devices uses specialised optics to display objects within the user's FOV. The special optics are configured in such a way to allow light to pass through and still let the users see their physical surroundings unlike the displays on the video see-through types. Vuzix teamed up with Nokia to release a set of smart glasses (i.e. the M2000AR, Blade 3000, M3000, and AR3000) \cite{vuzixwaveguide} that utilises \textit{waveguide optics} but we are yet to see these devices come out in the market. One of the most popular HMD devices using optical technology is the Google Glass that uses a semi-transparent prism on which projected images are reflected towards the eye \cite{olsson2013wearable}. However, the Google Glass does not perform object tracking which makes its functionality very similar to that of the Recon Jet and the Vuzix smart glasses -- as an eye wear version of a smart watch.

Nonetheless, there are already numerous optical see-through HMD devices that performs object tracking and allows users to interact with synthetic objects augmented on the physical world. Epson's Moverio BT-300\footnote{Moverio BT-300 Smart Glasses (AR/Developer Edition), (Accessed 4 Aug 2017), https://epson.com/For-Work/Wearables/Smart-Glasses/Moverio-BT-300-Smart-Glasses-\%28AR-Developer-Edition\%29-/p/V11H756020} provides binocular visual augmentations using a similar prism projection mechanism and accepts user inputs using a capacitive muti-touch pad tethered to the eye-wear. ODG's R7\footnote{R-7 Smartglasses System, (Accessed 4 Aug 2017), https://shop.osterhoutgroup.com/products/r-7-glasses-system} smart glasses is another optical see-through device but accepts user inputs using conventional approaches, i.e. mouse and keyboard. DAQRI's HMDs utilises a bi-phasic crystal element\footnote{Software defined light. (Accessed 4 Aug 2017), https://daqri.com/technology/software-defined-light/} that can change its optical properties, which effectively changes how light is perceived by the eyes, by using electric fields instead of the regular prism projection mechanism and, to some extent, detects user input in order to interact with the augmented virtual objects. %\cite{daqritheverge}. 

In terms of natural user gesture support, the leading devices are the Meta 2 glasses and Microsoft's Hololens. The Meta 2\footnote{The Meta 2: Made for AR App Development, (Accessed 4 Aug 2017), https://buy.metavision.com/}delivers 3D holographic objects and utilizes environment tracking to allow a virtual 360\degree interface, and allows users to drag, pull, and drop objects within the space. However, it is tethered to a dedicated machine which has to have a dedicated graphics processor. Microsoft's HoloLens provides a similar experience to that of the Meta 2 but untethered. In early 2016, Microsoft started shipping out developer editions, and they expect that developers will create numerous services and applications around the HoloLens \cite{hololens}. %The Hololens \footnote{HoloLens hardware details, (Accessed 4 Aug 2017), https://developer.microsoft.com/en-us/windows/mixed-reality/hololens_hardware_details/} packs two high-definiton light engines, holographic lenses, an inertial measurement unit (IMU), 4 environment understanding cameras, a depth camera, and a dedicated holographics processing unit aside from the regular hardware (e.g. processor, memory, and battery) that the other devices have. Obviously, the cost for being untethered is the battery performance which is only 5.5 hours maximum and halves at heavy load \cite{hololensbattery}.

\subsubsection{Other form factors}
However, most of those devices mentioned above require that they be worn or held by the users which can bring user discomfort. Other projective form factors can provide MR functionalities without the burden of HMDs. \textsc{Lampix} is a smart lamp that uses a projector and a camera to transform any surface into an interactive surface \cite{lampix}. Sony \cite{xperiatouch} also provides a similar projective device that turns any surface into a smart phone interface allowing users to interact with the projections just like in a smart phone. \textsc{Lampix} goes further by detecting other objects (e.g. physical documents, coffee pods, etc.) that are placed within its view and allows these objects to interact with the projected objects.

Aside from the devices above which are primarily designed around the user, i.e. creating services literally surrounding the user, there are also other form factors that are designed for specific tasks such as the AR head-up displays (HUD) that are installed on cars usually on the dashboard. In recent years, various car manufacturers have incorporated these HUDs that provides drivers with assistive information such as lane departure warnings, adaptive cruise control, or navigation directions \cite{bbccarhud2014}. Now, manufacturers are also considering of adding more functionalities such as showing social media feeds. Continental\footnote{Head -up Displays, (Accessed 4 Aug 2017), http://continental-head-up-display.com/} provides two types of HUDs: a reflective HUD using reflections to the windshield, and a combiner HUD. Panasonic brings in more object detection, such as pedestrians, and visual information, such as camera feed from different directions which effectively eliminate the need for side mirrors \cite{dashboardAR}. DAQRI is also bringing their optical technology to vehicular HUDs\footnote{DAQRI SMART HUD, (Accessed 4 Aug 2017), https://daqri.com/products/smart-hud/}.

\subsection{Security and privacy of these devices, platforms, and applications}\label{sec:risks}

%Clearly, major technology companies are providing support in driving MR to reality. Google has made a significant financial contribution to the (still mysterious) company MagicLeap, which aims to deliver another MR HMD that will blur the real from the virtual \cite{magicleap}. Even content and social media companies are also joining the trend with expectations that MR will enable new forms of content and that it will definitely be social \cite{facebookVR}. Due to these thrusts of support, it is expected that MR devices will compete with or most likely replace the smart phone as our daily driver. We have already seen this trend even with just the smart watches we have now.

%There have already been various security and privacy work on MR-related technologies. Several of these are targetted towards sensor management, wearable devices, and personal data protection, as well as a few on AR. For example, potential long-term solutions for the different security and privacy risks associated with using AR browsers, e.g. Wikitude and Layar, have been proposed \cite{McPherson2015ARBrowsers}; however, no actual prototypes were evaluated. Thus, on the succeeding subsections, we will expound on the different approaches that have been proposed and evaluated, and discuss how their implementations varied.

Moreover, the current MR devices and platforms now provides a peak on what the future devices will offer. Given the capabilities of these devices, both in sensing and display rendering, there are numerous concerns on security and privacy that have been raised and needs to be addressed \cite{conti2013malicious,dwight2016risks,tynan2017hacker}. In fact, real vulnerabilities have already been revealed particularly on the numerous released applications. For example, Pokemon Go's network messages between the application and their servers on its early releases were vulnerable to man-in-the-middle attacks \cite{colceriu2016catching} which allows hackers to get precise location information of users. In addition to these were the numerous malicious versions of the application \cite{burgess2016pokemongo,frink2016pokemongo} that has been downloaded and used by many users. 

Apart from those, there have been no security and privacy analysis or assessment of these commercially-available devices and platforms. There was an effort that pinpointed risks and identified long-term protection for AR browsers, i.e. Wikitude, Layar, and Junaio, \cite{McPherson2015ARBrowsers} but no actual nor systematic evaluation was done on both the risks and the proposed protection. In the following sections, we will discuss the various security and privacy approaches that have been proposed in the literature for MR and related technologies and present a categorization of these approaches.



==> summary_table.tex <==
\begin{table}[]
	\centering
	\caption{Summary of all approaches that have been discussed, and which security and privacy controls are applied by each approach and to what extent.}
	\label{tab:approaches}
	\small
	\begin{tabular}{@{}p{3.8cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}@{}}
		\toprule
		\textbf{Approaches}                               & \textbf{AC}     & \textbf{DM}    & \textbf{AU}    & \textbf{DA}    & \textbf{MP}    & \textbf{MA}    & \textbf{MS}    & \textbf{S}     & \textbf{PA}    & \textbf{IS}    & \textbf{TC}    & \textbf{CP}    & \textbf{DP}    & \textbf{OC}    \\ \midrule
		\multicolumn{15}{c}{{\small Input Protection Approaches}}                                                                                                                                                                                                                                                 \\ \hline
		\cite{jana2013scanner}$\ddagger$                            & $\blacksquare$* & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{zarepour2016context}$\ddagger$                        & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{templeman2014placeavoider}$\dagger$                  & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{szczuko2014augmented}$\otimes$                       & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{wang2017scalable}$\otimes$                           & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{truong2005preventing}$\otimes$                       & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\boxplus$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{hayashi2010installation}$\ddagger$                    & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$      & $\square$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{roesner2014world}$\ddagger$                           & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      \\
		\cite{aditya2016pic}$\dagger$                              & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{li2016privacycamera}$\dagger$                        & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{shu2016cardea}$\dagger$                              & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{raval2014markit,raval2016you}$\dagger$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{forte2014eyedecrypt}$\ddagger$                        & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\blacksquare$ & $\blacksquare$ & $\blacksquare$ & $\boxplus$    & $\boxplus$    \\
		\cite{maiti2017preventing}$\ddagger$                        & $\square$  & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{figueiredo2016prepose}$\ddagger$                     & $\blacksquare$* & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{jana2013enabling}$\ddagger$                           & $\blacksquare$* & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\boxplus$    & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\ \hline
		\multicolumn{15}{c}{{\small Data Protection Approaches}}                                                                                                                                                                                                                                                 \\ \hline		
		\cite{sweeney2002k}$\otimes$                               & $\square$       & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{dwork2014algorithmic}$\otimes$                       & $\square$       & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{mcsherry2007mechanism}$\otimes$                      & $\square$       & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{erlingsson2014rappor}$\otimes$                       & $\square$       & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{xu2015semadroid}$\otimes$                            & $\blacksquare$  & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{huang2011faster}$\otimes$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\square$      \\
		\cite{gentry2009fully}$\otimes$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\square$      \\
		\cite{sekhavat2017privacy}$\ddagger$                        & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\square$      \\
		\cite{mun2010pdv}$\otimes$                                 & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\square$      \\
		\cite{deMontjoye2014openpds}$\otimes$                      & $\square$       & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\blacksquare$ & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      \\
		\cite{crabtree2016databox}$\otimes$                        & $\square$       & $\square$      & $\blacksquare$ & $\square$      & $\boxplus$    & $\blacksquare$ & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      \\ \hline
	\end{tabular}
	%\tiny
	\begin{tabular}{p{0.95\textwidth}}
		The security and privacy controls are labelled as follows: \textbf{AC} = Access Control Policy; \textbf{DM} = Data Mining Protection; \textbf{AU} = Audit and Reporting; \textbf{DA} = Device Authentication; \textbf{MP} = Media Protection Policy; \textbf{MA} = Media Access; \textbf{MS} = Media Storage, Storage Protection, and Boundary Protection; \textbf{S} = Media Sanitization; \textbf{PA} = Physical Access Control, and Access to Output Devices; \textbf{IS} = Information in Shared Resources, Information Sharing; \textbf{TC} = Transmission Confidentiality and Integrity; \textbf{CP} = Cryptographic Protection, Key Establishment and Management, and/or PKI certificates; \textbf{DP} = Distributed Processing and Storage; \textbf{OC} = Out-of-band Channels.\\
		* Least privilege is applied to \textbf{AC}. \\
		The extent of each control was $\blacksquare$ fully applied, $\boxplus$ partially applied, or $\square$ not applied or mentioned.\\
		The controls have been applied to a $\ddagger$ MR context, $\dagger$ proto-MR context, $\otimes$ non-MR context.
	\end{tabular}
\end{table}
\addtocounter{table}{-1}
\begin{table}
	\centering
	\caption{(\textit{Continuation}) Summary of all approaches that have been discussed, and which security and privacy controls are applied by each approach and to what extent.}
	\small
	\begin{tabular}{@{}p{3.8cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}p{.35cm}@{}}
		\toprule
%		& \multicolumn{14}{c}{\textbf{Security and Privacy Control Used}}   \\ \cline{2-15}  
		\textbf{Approaches}                               & \textbf{AC}     & \textbf{DM}    & \textbf{AU}    & \textbf{DA}    & \textbf{MP}    & \textbf{MA}    & \textbf{MS}    & \textbf{S}     & \textbf{PA}    & \textbf{IS}    & \textbf{TC}    & \textbf{CP}    & \textbf{DP}    & \textbf{OC}    \\ \midrule
		\multicolumn{15}{c}{Output Protection Approaches} \\ \hline
		\cite{eaddy2004my}$\ddagger$                                & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{woo2012vrcodes}$\ddagger$                             & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{lin2017video}$\ddagger$                               & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{lantz2015visual}$\ddagger$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\boxplus$      & $\square$      & $\square$      \\
		\cite{andrabi2015usability}$\ddagger$                       & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\boxplus$      & $\square$      & $\square$      \\
		\cite{fang2010securing}$\ddagger$                           & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\blacksquare$ & $\boxplus$      & $\square$      & $\square$      \\
		\cite{lebeck2016safely, lebeck2017securing}$\ddagger$                           & $\blacksquare$  & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{vilk2014least, vilk2015surroundweb}$\ddagger$                              & $\boxplus$*     & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\ \hline
		\multicolumn{15}{c}{Interaction Protection Approaches}   \\ \hline
		\cite{butz1998vampire, butz1999emmie}$\ddagger$             & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{devincenzi2011kinected}$\ddagger$                     & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{reilly2014secspace}$\ddagger$                         & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{ens2015candid}$\otimes$                             & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\boxplus$    \\
		\cite{szalavari1997personal, szalavari1998gaming}$\ddagger$ & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{cheok2002touch}$\ddagger$ & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{xu2008bragfish}$\ddagger$                             & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\boxplus$    & $\square$      \\
		\cite{gaebel2016looks}$\dagger$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\blacksquare$ & $\square$      & $\blacksquare$ \\ \hline
		\multicolumn{15}{c}{Device Protection Approaches}  \\ \hline
		\cite{george2017seamless}$\ddagger$                        & $\square$       & $\square$      & $\square$      & $\boxplus$    & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{aslan2014mid}$\dagger$                               & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{rogers2015approach}$\dagger$                         & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{li2016move}$\ddagger$                                 & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{venkatasubramanian2010pska}$\otimes$                 & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      \\
		\cite{schneegass2016skullconduct}$\dagger$                 & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{raja2015multi}$\dagger$                              & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{khamis2016gazetouchpass}$\dagger$                    & $\square$       & $\square$      & $\square$      & $\blacksquare$ & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{kohno2016display}$\ddagger$                           & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$    & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{mollers2011taps}$\otimes$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$    & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      \\
		\cite{pearson2017chameleon}$\otimes$                            & $\square$       & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\square$      & $\blacksquare$    & $\square$      & $\square$      & $\square$      & $\square$      & $\square$ \\ \bottomrule
	\end{tabular}
	\begin{tabular}{p{0.95\textwidth}}
		The extent of each control was $\blacksquare$ fully applied, $\boxplus$ partially applied, or $\square$ not applied or mentioned.\\
		The controls have been applied to a $\ddagger$ MR context, $\dagger$ proto-MR context, or $\otimes$ non-MR context.
	\end{tabular}
\end{table}
\textsl{}
